Building an Emulation Environment for Cyber Security Analyses of Complex Networked Systems

Computer networks are undergoing a phenomenal growth, driven by the rapidly increasing number of nodes constituting the networks. At the same time, the number of security threats on Internet and intranet networks is constantly growing, and the testing and experimentation of cyber defense solutions requires the availability of separate, test environments that best emulate the complexity of a real system. Such environments support the deployment and monitoring of complex mission-driven network scenarios, thus enabling the study of cyber defense strategies under real and controllable traffic and attack scenarios. In this paper, we propose a methodology that makes use of a combination of techniques of network and security assessment, and the use of cloud technologies to build an emulation environment with adjustable degree of affinity with respect to actual reference networks or planned systems. As a byproduct, starting from a specific study case, we collected a dataset consisting of complete network traces comprising benign and malicious traffic, which is feature-rich and publicly available.

==> related_work.tex <==
%!TEX root = ./main.tex
\section{Related Work}


\mara{TODO: Qui io parlerei del progetto PANOPTESEC}

\paragraph{Tools for creating emulated environments}

\mara{Terraform}
In~\cite{eskridge2015vine} the authors proposed a Virtual Infrastructure for Network Emulation (VINE), pointing out for a set of tools that helps the construction of virtual topologies allowing for different type of experiments for cyber security researchers. %In particular, they provide three topology-generation methods: manual, programmatic, and tool-based. 
Furthermore, VINE supports traffic behavior generation using monitored agents or the traditional packet capture for a low-level analysis of the state of the hosts. Operators can exploit a web-based interface, to manually create, modify, and monitor experiment testbeds as well as a JSON HTTTP interface for automated generation and control experiments. The main drawback of this paper is that the platform is overviewed at a rather general viewpoint, without allowing for a deep comparison.

\sncs{As cybersecurity work, the authors in ~\cite{Pham2016CyRISAC} proposed a Cyber Range Instantiation System (CyRIS). It is a solution of reliably and repeatably creating and managing environments for cybersecurity training courses. In particular, CyRIS is an automated tool that takes a cyber range definition description (a file)and creates the desired training environments without human interaction. Furthermore, it supports both basic features for preparing the infrastructure, and security features for configuring sophisticated security related content.}

\paragraph{Mapping a reference environment}
%[Raniero]'s paper 
All considered tools provide means for security testbeds instantiation and experimentation, and either concentrate on Most papers concentrate either of . Our work documents instead a complete end-to-end methodology mapping an existing real environment inside an emulated environment, and performing cyber security experiments.
Previously, ~\cite{raniero18} Rapone et al. concentrated of the latter aspect, on providing a measurable metric for determining the affinity of a virtual environment with respect to the reference real environments.
\mara{Il paper di Raniero sembra piu un technical report (non pubblicato, presente solo su researchgate). Valutiamo se ometterlo.}



%\paragraph{Works on Network intrusion dataset collections}
We refer to more related work in each of the following sections.

==> technical report/conclusions.tex <==
%Nelle conclusioni evidenziare anche questo problema aperto
\section{Conclusions and Future Work}
This paper proposes a methodology for the design, development and deployment of cloud-based emulation environments.
Based on our practical experience, we provided some recommendation about technological choices to support the creation of virtual environments.
We also show the effectiveness of our approach by applying our methodology to build an emulation environment for the study case of our Department network.
Finally, we show the flexibility of the deployed environment to simulate actual cyber attacks and benign traffic, that we collected in a publicly released dataset containing complete network traces, enriched with labeled features.
%This paper represents a first step towards the definition of an environment able to support cyber security testing and training activities.
%There are however some limitations that we considered along the definition of our methodology. Since the focus of this work was on open-source software, a general lack of documentation and error reports were a fact, which extended some effective open research problems in this area of study. In particular, for the automation of installed services needs an improvement for the CPE management. Accordingly, software vendors (including free software authors and proprietary vendors) should include a list of CPE describing the software included in their distributions to support the work of people and organization who try to do vulnerability management version services assessment.
A limitation of our work is the lack of an evaluation of the accuracy of the information acquired from the reference network mapping phase, due to lack of precise ground truth, which would require an intrusive approach. 
As a future step in this direction, we plan to work on the definition of a strategy to measure the affinity of the final emulated environment and the original reference network. 
%Furthermore we committed to using only open source software, while important alternatives exist, both in the cloud environment and in the network scanning software landscape.
The next step in our investigation will be toward the definition of novel approaches to develop user behavior profilers to improve the quality of benign data generators in terms of closeness to real human behavior.
Additionally, we plan to investigate approaches to fully automate the installation of services, which is currently an open issue.
%Indeed, the CPE management could be slightly improved with a collaborative approach to add or updates CPE entries. Therefore, software vendors (including free software authors and proprietary vendors) should include a list of CPE describing the software included in their distributions to support the work of people and organization who try to do vulnerability management version services assessment.

%\mara{Problema aperto, mapping CPE - applicativi installati}




==> technical report/dataset.tex <==
\section{Dataset}
As part of our work, we gathered a realistic dataset, comprising of benign and malicious traffic, that has been processed to obtain feature-rich labeled attack flows, useful for cyber security analyses such as training IDS and IPS classifiers and other machine-learning tasks, as well as for deep packet inspection investigation and related activities.
In particular, the following sections elaborate on our benign profile agents and the a number attack scenarios that we considered.

\subsection{Benign Traffic Agents}
\label{sec:dataset_generators}
To form the main part of our dataset, out aim was having realistic background traffic that comprises a number of widely used protocols, namely HTTP, HTTPS, SSH, SMB and SFTP, to act as background noise with respect to a number of traffic flows corresponding to specific instantiated attack patterns. To this end, we used a number of software agents written in Python to provide close-to-realistic user behavior for the VLANS from LAN1, through LAN4.\\
The agents' software consists in a number of traffic simulation jobs executed by worker threads managed by a scheduler, which feeds the threads following a specific \emph{traffic profile} shown in Table~\ref{tab:dataset_traffic_profile}), and assigned to each machine. In particular, on average, each job will be executed during the interval (Start, End) defined in the profile, a number of times depending on the Frequency profile.
The scheduler will randomize the time between the execution of each job to 
prevent the traffic from looking too synthetic.  
Furthermore, all jobs have an initial setup phase that always entails a degree of randomness in all configurable parameters, as well as multipliers for randomly delaying each request.\\

In the following, we summarize the behavior of the simulation jobs for the different protocols supported by our agents.\\\\
\textbf{HTTP/HTTPS generator:}  
An HTTP job, ``browses'' the internet starting at pre-defined root urls and simulates clicks by randomly following links on pages until a pre-defined click depth of 7 is met. Wait time between HTTP requests is chosen at random uniformly between 5 and 10 seconds.
    The number of total http requests is given by a random integer generated uniformly between 1 and of 20. The value of the parameters has been chosen following previous research~\cite{wang2004characterizing,white2007investigating}, that found that only about 5\% of sessions are longer than 20 requests and the average session length is about 7. Note that to generate request that are compatible with the associated OS, each agent will perform requests with a specific \texttt{User-Agent} that is automatically identified by the software based on the machine OS.\\\\
\textbf{SSH generator:} 
An SSH job connects to a host with the provided credentials using SSH and start sending commands selected at random from a list of supplied commands, keeping the connection open until a given period of time generated at random. 
The commands list is generated at startup time from a list of common commands such as \texttt{`ls', `cd', `cat /var/log/messages'}, etc.\\\\
\textbf{SMB generator:}
A SMB job connects to a SMB share with the provided credentials and uploads and downloads a number of files or directories. The files are randomly generated and their size are controlled by an optional size multilier of the default size of 8192 bytes.\\\\
\textbf{SFTP generator:} An SFTP generator connects to a host with the provided credentials using the SSH subsystem SFTP. It then starts uploading and downloading files provided with the same parameters of the SMB generator.

\begin{table}[]
\centering
\begin{tabular}{|c|r|r|r|c|c|llll}
\cline{1-6}
\textbf{Type} & \multicolumn{1}{c|}{\textbf{Start}} & \multicolumn{1}{c|}{\textbf{End}} & \multicolumn{1}{c|}{\textbf{Freq}} & \textbf{Hosts} & \textbf{Servers}       &  &  &  &  \\ \cline{1-6}
WEB           & 9:00                                & 18:30                             & 15                                 & All            & *                      &  &  &  &  \\ \cline{1-6}
SMB1          & 9:00                                & 18:00                             & 60                                 & All but h2     & lsrv                 &  &  &  &  \\ \cline{1-6}
SMB2          & 14:00                               & 18:00                             & 180                                & All but h2     & lsrv                 &  &  &  &  \\ \cline{1-6}
SSH3          & 9:00                                & 18:00                             & 60                                 & h1             & ced2                   &  &  &  &  \\ \cline{1-6}
SSH4          & 9:00                                & 18:00                             & 240                                & h2             & lsrv, ced1-3, int1-3 &  &  &  &  \\ \cline{1-6}
SSH5          & 9:00                                & 18:00                             & 60                                 & h3             & ced3                   &  &  &  &  \\ \cline{1-6}
SSH6          & 9:00                                & 18:00                             & 60                                 & h4             & int1                   &  &  &  &  \\ \cline{1-6}
SSH7          & 9:00                                & 18:00                             & 60                                 & h5             & int2                   &  &  &  &  \\ \cline{1-6}
SFTP          & 9:00                                & 18:00                             & 240                                & All but h2     & int3                   &  &  &  &  \\ \cline{1-6}
\end{tabular}
\caption{Traffic generator profiles for the various supported protocols. All, refers generically to all hosts in the four business VLAN1-4. The reported custom hosts correspond to: h1 (10.1.10.9), h2 (10.1.10.8), h3 (10.1.10.17), h4 (10.1.10.13), h5 (10.1.11.3).}
\label{tab:dataset_traffic_profile}
\end{table}

%\mara{TODO: spiegare in breve qual'e l'idea dietro ai behavior, in particolare degli host con comportamento custom.}

The agents' code has been deployed at machine instantiation time using init scripts, and the resulting processes are configured as Systemd (Ubuntu 14.04+, Debian) or Upstart Jobs (Ubuntu until 14.04), and using Task Scheduler on all Windows OS, configured to run as automatic startup jobs and to be automatically restarted in case of failures.


==> technical report/dataset_attacks.tex <==
\subsection{Attack profiles and scenarios}
\label{sec:attack_scenarios}
To give a practical demonstration of the power and flexibility of our emulated environment, we performed various cyber attacks in the testbed, covering a diverse set of attack scenarios. In particular, starting from common attack taxonomies, 4 attack profiles were selected, and executed by using related tools and codes.\\\\
\textbf{Brute Force:}
A brute force attack can target different types of services. The main goal of this attack is obtaining private information, \ie a password, or private key, by testing many input combinations through a trial and error process, until the private information is finally gathered. This attack is one of the easiest to perform and detect, given the huge amount of traffic generated by the probing process. 
In particular, we performed a Dictionary-based brute-force attack to an OpenSSH daemon running on a Linux Machine.\\\\\
\textbf{Heartbleed:}
Heartbleed is a vulnerability of the OpenSSL implementation of the SSL protocol. The name comes from a specific function introduced in version 1.0.1, called \emph{HeartBeat}: this extension allows the clients to test and keep a connection alive without the need of re-negotiating it from scratch. Thus, suffering from a buffer-over-read vulnerability, it allows the clients to read more data than expected, possibly leaking sensitive information. To perform this attack, an SSL connection must be instantiated with a vulnerable server, sending a malformed Heartbeat request.\\\\
\textbf{Web Application Attack:}
Attacks on web applications may target different services. The OWASP Top 10~\footnote{\url{https://www.owasp.org/index.php/Top_10-2017_Top_10}} shows the most common pattern for this specific attack surface, where the targets span from simple websites to complex CMS. As a practical case, we targeted the Drupal CMS version 7.31, vulnerable to a Remote Command Execution (RCE) exploit called drupalgeddon2 (CVE 2018-7600). With this attack, it is possible to obtain control of the attacked server by exploiting a sanitization vulnerability in the AJAX requests %composed of Drupal Form %API’s renderable arrays, used to render a requested page through Drupal’s theming system. Through four specific rendering functions, 
allowing the attacker to force the vulnerable server to execute arbitrary malicious code.\\\\
\textbf{LAN Attack (+ Ransomware Deployment):}
This attack pattern was introduced to represent an insider threat, \ie a malicious user who has access to the organization's internal network. We conducted a lateral spreading attack by exploiting an SMB vulnerability (CVE-2017-0144) affecting various Microsoft Windows versions, as made by the Eternalblue exploit used in 2017 for spreading the DoublePulsar backdoor. In this case, the attack started from an intruder Kali Linux, connected to the LAN1. The attack begins with a series of Nmap scans (alive, services) towards LAN4, where a victim is found having a vulnerable Windows 7 system. The attacker installs a reverse TCP shell via Eternalblue and using a local HTTP server installed on the attacker machine downloads and runs the famous WannaCry software on the victim machine.\\
%More information on the exploits can be found on Exploit-db~\footnote{\url{https://www.exploit-db.com}}.

%Once executed, the WannaCry ransomware encrypts all files with matching a list of extensions, then changing the background image of the infected host by explaining what happened and how the user could get his file back. To decrypt the files, the user should pay the ransom by sending a given amount of bitcoins to a bitcoin wallet: once the payment has been successful, if the attacker keeps his word, the victim receives the decryption key to restore his files. 
All the specific attack steps as well as the corresponding timeline will be publicly released along with the full capture dataset. 


==> technical report/dataset_data_collection.tex <==
\subsection{Data Collection}
Our data collection objective was gathering full traffic capture for all VLANs pertaining to the department network infrastructure, namely LAN1 through LAN4, FWVR0, FWVR1, as well as the service LANs CED, DMZ\_INT and DMZ\_EXT. 
%To recall, each VLAN sits on a specific bridge, yet VMS can span all server nodes and have interfaces in different VLANs. 
\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{|l|r|r|c|r|r|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{Attacker}} & \multicolumn{1}{c|}{\textbf{Victim}} & \textbf{Day} & \multicolumn{1}{c|}{\textbf{Start}} & \multicolumn{1}{c|}{\textbf{End}} & \multicolumn{1}{c|}{\textbf{Time (s)}} & \multicolumn{1}{c|}{\textbf{\# pkts}} & \multicolumn{1}{c|}{\textbf{Avg. pps}} & \multicolumn{1}{c|}{\textbf{Avg. size (B)}} \\ \hline
\textbf{Heartbleed}                 & 1.2.3.3                                & 200.100.0.8                          & \textbf{25}  & 15:01:51                            & 15:06:08                          & 256.3                                  & 144                                   & 0.6                                    & 720                                         \\ \hline
\textbf{Bruteforce}                 & 1.2.3.3                                & 200.100.0.3                          & \textbf{25}  & 16:03:37                            & 17:59:13                          & 6935.5                                 & 504641                                & 72.76                                  & 137                                         \\ \hline
\textbf{Web}                        & 1.2.3.16                               & 200.100.0.3                          & \textbf{27}  & 10:39:05                            & 11:06:50                          & 1665.2                                 & 554                                   & 0.33                                   & 581                                         \\ \hline
\textbf{LAN}                        & 10.1.10.2                              & 10.1.12.2                            & \textbf{27}  & 12:21:30                            & 12:40:57                          & 1167.5                                 & 2816                                  & 2.41                                   & 1464                                        \\ \hline
\textbf{PortScan}                   & 10.1.10.2                              & LAN4                                 & \textbf{27}  & 12:07:32                            & 12:21:30                          & 838                                    & 24388                                 & 29.10                                  & 61                                          \\ \hline
\end{tabular}

\caption{Time and statistics for the attack instances deployed in the testbed. Times are in  CEST timezone}
\label{tab:attacks_stats}
\end{table*}

Following the directions discussed in Section~\ref{sec:meth_data_coll}, to perform the full traffic capture, we deployed a sniffer VM for each pair $(n, b)$ (where $n$ is a node and $b$ is an OVS bridge) having one network interface on each VLAN $v$ belonging to bridge $b$. Each of such port has been configured to be the output port of a SPAN mirror, that receives traffic from all interfaces of VLAN $v$, belonging to machines deployed on node $n$. We thus captured traffic from all sniffers network interfaces using the Linux network traffic capturing tool \texttt{tcpdump}.

 %However, since br1 contains networks where the virtual machines can communicate with each other, we have a duplicate for each traffic between two VMs in two different specific VLAN. This is due by capturing the traffic for each VLAN. We removed these duplicates with a post-processing technique. 

The data capturing period started at 14:30 on 25 July 2018 and continuously ran for an exact duration of 4 days, ending at 14:30 on 29 July 2018. 

\noindent As described in the previous section, it contains both benign traffic generated with our agents as well as malicious traffic flows. Concerning the latter, we deployed some instances of the attack profiles reported in Section~\ref{sec:attack_scenarios} and extracted the corresponding network traffic from the captures to obtain a list of attack-traffic subcaptures. Statistics for each attack are shown in Table~\ref{tab:attacks_stats}, \ie involved hosts, attack timespans (start, end and duration), total number of packets, average packets per second and average packet size in bytes.
The PortScan row refers to the Nmap scanning phase of the LAN Attack scenario.
Furthermore, we processed all attack-traffic captures with a flow-based feature extractor~\cite{lashkari2017characterization,sharafaldin2018toward}, in a way to extract 80 features for all included flows, where each flow corresponds to a \texttt{(SrcIP, SrcPort, DstIP, DstPort,Protocol)} tuple.
The extracted features are useful for training Intrusion Detection and Prevention Systems (IDS, IPS) classifiers and other machine-learning tasks for cyber security analyses~\cite{sharafaldin2018toward}.\\
\noindent To summarize, the dataset~\footnote{The full dataset is available at \url{https://www.cis.uniroma1.it/dataset_ICDCN2019}, released under the CC-BY license.} contains the following information:\\
\begin{itemize}
\item \textbf{Full daily captures:} One PCAP file per day with the full capture for each VLAN.
\item \textbf{Attacks:} A separated PCAP files for each attack, as per Table~\ref{tab:attacks_stats}, a well as a description of the necessary steps to replicate it.
\item \textbf{Benign:} A separate PCAP file with all traffic from LAN1-LAN2 for 26/07, containing only benign (agent-related) flows, as per Table~\ref{tab:dataset_traffic_profile}).
\item \textbf{Features:} for each PCAP file, a CSV files containing, for each extracted flow, the values for 80 traffic related features.
\end{itemize}




==> technical report/intro.tex <==
%!TEX root = ./main.tex
\section{Introduction}

\noindent {\bf Context and Motivation.} Starting from the past decade, cyber attacks have become increasingly sophisticated, stealthy, targeted and multi-faceted, featuring zero-day exploits and highly creative interdisciplinary attack methods.
Furthermore, it is most likely an upward trend, due to two main factors: (i) increasing complexity of ICT networks and (ii) increasing capabilities of cyber attackers.
%that are becoming always more smart.
As a consequence, cyber security is becoming of primary importance for every organization, including small and medium enterprises and large companies, as well as critical infrastructures on which our society is becoming increasingly dependent.
%on (critical) cyber infrastructure.

One of the countermeasures that can be taken to face attackers is to try to play the role of the attacker and stress the environment that is aimed to protect. However, in order to enable this possibility, a separate, dedicated emulation/simulation environment must be set in place. 
Such environment should be able to: (i) represents realistic cyber environments that fit the testing objectives, (ii) offer tools for producing both benign and malicious system events and (iii) support the definition and creation of new scenarios and cyber threats in a cost and time-effective manner~\cite{eskridge2015vine,pham2016cyris}.

Combining network and security assessment techniques with the use of cloud technologies allows for the deployment of emulation environments.
The objective of an emulation environment is enabling the deployment of fully virtualized instances of computer networks, with adjustable degree of affinity with respect to an actual reference networks or planned systems~\cite{raniero18}, allowing for arbitrary speculative analyses, notably for what concerns cyber security.\\



\noindent{\bf Related Work.} %Many tools provide means for security testbeds instantiation and experimentation. However, they support particular needs and are not general enough.
To the best of our knowledge, currently, very few complete solutions exist to support the design, development and deployment of an emulation environment to support testing and training.
In~\cite{eskridge2015vine} the authors proposed a Virtual Infrastructure for Network Emulation (VINE), pointing out for a set of tools that helps the construction of virtual topologies allowing for different type of experiments for cyber security researchers. %In particular, they provide three topology-generation methods: manual, programmatic, and tool-based. 
Furthermore, VINE supports traffic behavior generation using monitored agents or the traditional packet capture for a low-level analysis of the state of the hosts. Operators can exploit a web-based interface, to manually create, modify, and monitor experiment testbeds. %as well as a JSON HTTP interface for automated generation and control experiments. 
The main drawback of this paper is that the platform is overviewed at a rather general viewpoint, without allowing for a deep comparison.
In the specific context of cybersecurity, in ~\cite{pham2016cyris}, the Cyber Range Instantiation System (CyRIS) system is presented, as a solution, based on OpenStack, for reliably and repeatably deploying cyber ranges, \ie, technology development environments for cybersecurity training courses. 
%It consists of an automated tool that takes a file containing a cyber security definition description and creates the desired training environments without human interaction. 
It supports basic automation for systems and network deployment, and a certain degree of automation for sophisticated security activities (such as modifying firewall rules or planting malware). Another, close-sourced example is~\cite{yasuda2016alfons}. 
%\maraedit{
While these works provide valid tools for deploying testbeds for cyber experimentation, none of them tackles the task of documenting a methodological framework for creating emulation environments (along with the multiple existing technical tradeoffs).
Our paper, instead, presents a complete end-to-end methodology to build a virtual environment and deploying a cyber security testbed, mapped from an existing network. Furthermore, our work directly shows the benefit of the approach by providing a realistic dataset which can benefit multiple sides of the cyber-security scientific community.\\



\noindent {\bf Contributions.}
This paper provides three main contributions: (i) it proposes a methodology for designing and deploying a cloud-based emulation environment, (ii) it discusses the application of the proposed methodology to a case study and (iii) it shows the flexibility and power of the proposed approach to build an environment that is able to generate a realistic dataset, comprising of benign and malicious traffic. Furthermore, the dataset has been processed to obtain feature-rich labeled attack flows, useful for cyber security analyses such as training IDS and IPS classifiers and other machine-learning tasks, as well as for deep packet inspection investigation and related activities.
%the lessons learnt 
In particular, we exploit our practical study case to highlight, for each step of the methodology, how the relevant technologies and tools can be combined to achieve specific design requirements in an effective way.
%that can be used to define novel approaches (possible based on machine learning techniques) for the detection of cyber attacks and for testing the effectiveness of novel mitigation strategies.


%The rest of the paper is organized as follows. In Section 2 some background for our work is provided. In Section 3 . The results of .. are presented in Section 5, together with . Finally, some conclusions and future directions for our work are outlined in Section 5.

%\mara{TODO: Qui va un cappello sulla cybersecurity e sui concetti di simulation vs emulation (i.e. simulazione dello stato interno dei vari componenti vs solo comportamento esterno) allo scopo di fare ricerca in cybersecurity, dicendo che noi ci limitiamo a realizzare un environment che permette di fare analisi di vulnerabilit e strategie a livello software e non hardware}




==> technical report/methodology_collection.tex <==

\subsection{Data Collection}
\label{sec:meth_data_coll}


To wrap up all information concerning the communication layer from Section~\ref{sec:meth_env_comm}, a testbed contains a number of virtual machines whose network interfaces belong to a number of VLANs sitting on a number of OVS bridges.
Layer3 routing between VLANs is handled by Virtual routers.In this section, we elaborate on different techniques and solutions for achieving network traffic data capture in an emulated testbed deployed in an emulation environment.\\\\
The problem of capturing and decoding traffic in high-speed network, be it physical or virtual has been deeply studied (see for example~\cite{braun2010comparing,fusco2010high}). In the context of a testbed for cyber security experimentation, the choice of a capturing solution depends on several criteria: reaction behavior, impact on network performance (delay, throughput), traffic rate and architectural considerations.\\\\
Typically, inline capture mode is preferred when the probe needs to react to intrusions (IPS) as it can alter or delete packets~\cite{kreibich2001network}. In particular, \emph{network taps} can be implied, \ie systems that are installed in network segments to monitor network devices such as % monitors events on a local network and in order to aid administrators (or attackers) in analyzing the network. When a tap is installed inline, it is present between two network devices. 
routers, firewalls, servers and hosts by means of network, application, or security analyzers, achieving high-speed full duplex capture with no data loss.
%The probe could also use this mode to normalize the capture traffic and thus to defend itself against evasion attacks. 
Inline capture mode might alter network performances due to packet processing delays, yet the analysis capacity of Next-Generation Intrusion Systems (NGIPS) in inline transparent mode has now reached speeds higher than the physical link, allowing for extremely low latencies~\cite{meena2018integrated}.
However, inline taps are only suited to monitor a point-to-point link, thus  not being a viable choice when the full data capture is of concern.
Moreover, an inline probe failure can induce network failures.

On the other hand, passive mode is stealthier and does not alter the performances or the availability of the monitored network. 
A cheap option is capturing on the hardware switches, yet VM-to-VM traffic that does not pass over a physical wire (e.g., if they are on the same VLAN on the same server) would not be captured.

Depending on the capturing requirements, thanks to its high flexibility and capabilities OVS can come to rescue.

As mentioned in Section~\ref{sec:meth_env_comm}, OVS bridges can help distributing the VLANs in logic compartments; this choice can also be made with data collection purposes in mind:
indeed deploying the VLANs on different bridges allows the sniffing in specific parts of the environment. 
However, even if the physical interface associated to each OVS bridge could be monitored, the issues related on same-node traffic is still present. 

When internal traffic of the VLANs is of concern (as, for example, if full capture is desired), OVS supports port mirroring capabilities (with the SPAN and RSPAN protocol)~\cite{pettit2010virtual}. For each network to be monitored, SPAN allows to mirror the traffic from all network interfaces toward a specific output port (the SPAN port). To achieve full capture the best option is to have a SPAN port for each bridge, for each physical node. Span output ports can be for example a network interface of a ``Sniffer'' VM, where the traffic is then collected to be later analyzed.

However, this solution can potentially suffer from bandwidth limitation and data loss, as the full traffic is replicated and sent to the sniffer.

\begin{figure}
	\centering 
	\includegraphics[width=\linewidth]{img/overview.pdf}
	\caption{Overview of the emulation environment testbed deployment and experimentation phases.}
	\label{fig:system_overview}	
\end{figure}

==> technical report/methodology_env.tex <==

\subsection{Virtual Environment Infrastructure}
\label{sec:meth_env}
%left low right up
\begin{figure*}
	\centering 
	\includegraphics[width=1\linewidth,trim={1cm 0cm 0.5cm 2cm},clip]{img/emulation_environment_infrastructure.pdf}
	\caption{Overview of the Emulation Environment infrastructure. An example configuration of the communication layer is reported, making use of three OVS bridges, namely \texttt{br1} (internal lans), \texttt{br2} (DMZ service lans) and \texttt{br3} (external lans).}
	\label{fig:meth_env_environment}	
\end{figure*}

In the following, we provide an overview of the main steps required to build up an emulation environment stack that fits our purposes of network emulation and cyber security experimentation.

%In particular Section~\ref{sec:meth_env_virt} starts reviewing the main available private cloud management platforms available, with particular reference to Infrastructure as a Service (IaaS) platforms and our framework of choice: OpenNebula. Then, various design choices will be discussed, such as the use of a distributed file system for the distribution of the virtual machine images among the compute nodes, and the communication stack. Following, Section~\ref{sec:meth_env_phys} describes the main involved logical pieces that help build the physical infrastructure.

\subsubsection{Private cloud Setup}
%Since the early 2000s, private clouds power companies and institutions with the ability to create software-defined networks and virtual machines, out of their own network infrastructure, in a very simple way.
%To this end, cloud management platforms are used, to manage and provide the storage ad compute resources provided by the physical infrastructure as a service. This is what gave the name to Infrastructure as a Service (IaaS) platforms, that allow accessing, monitoring, and managing datacenter infrastructures, providing end users with compute (virtualized or bare metal), storage, networking, and networking services (e.g. firewalls). 

Many IaaS platforms exist, and each one has its specific characteristics, furthermore, some platforms are constantly developing. 
The two major open-source ones by market penetration are OpenStack and OpenNebula, currently widely used by many people around the world~\cite{von2012comparison,vogel2016private}.
%\maraedit{
In order to set up our private cloud environment, we compared them taking into account the following features, namely \emph{Internal Organization, Software Deployment, Storage, Networking, Hypervisors and Governance}.
%
Due to lack of space, the detailed comparison with respect to the selected features is reported in Appendix~\ref{app:iaas_comp}.
%After the analysis and given our experience with them, OpenNebula is the suggest choice as it is a single open-source product, with a simpler usage and deployment.
After the analysis and experimentation with both, we found OpenNebula's solution both enterprise-ready and easy to use and deploy, thus being a good fit for any organization.  We chose OpenNebula as our IaaS for our case study (Section~\ref{sec:case_study}).
%}

\subsubsection{Storage and Distributed File System}
\label{sec:meth_env_dfs}
In a typical real environment, machines run various operating systems. 
On all cloud platforms, VM types have a corresponding notion of \emph{template}\footnote{Templates on OpenNebula documentation: \url{http://docs.opennebula.org/5.4/operation/vm_management/vm_templates.html}}: a collection of data (\ie a set of disk images) and metadata (\ie no. of associated cores, RAM, network interfaces, booting order, context information, etc).

Thus, typically when setting up an emulated environment, a proper template repository must be maintained, \ie a physical area where templates are stored, so that they can be easily browsed and recalled at VM instantiation time.
However, VMs can be instantiated on all physical nodes in the cluster, so a centralized repository would result in heavy load on the cluster (especially as such templates can be large, typically in the order of 20-100 Gbytes).
Therefore, a distribution or replication strategy could be implied.

GlusterFS (later, Gluster), is a scalable, distributed file system that aggregates disk storage resources from a pool of trusted storage servers into a single global namespace. It is used in production at thousands of enterprises spanning media, healthcare, government, education, web 2.0, and financial services~\cite{shirinbab2013performance}. A gluster \emph{volume} is a logical collection of export directories (called \emph{bricks}) located on the various servers of the pool. 
Various types of volumes are supported, and can be chosen depending on the distribution criteria that fits a specific use-case. To exploit data-locality at VM instantiation time, a good choice is setting up a \emph{Replicated GlusterFS Volume} %(Figure~\ref{fig:meth_env_gluster}). 

Apart for the inherent data redundancy, this solution also offers reliability as in case of a brick failure, the data can still be recovered from its replicas. 
Gluster supports LVM Volumes as mount points, so that multiple disks can be used for each server and regarded as a single volume. 
%Being a replicated fs, the size of the corresponding volumes must be identical on all machines.

%\sncs{GlusterFS uses the shared transfer driver that assumes that the datastore is mounted in all the hosts of the cluster. Furthermore, for shared filesystem datastore shared, where images are exported in a shared filesystem same solution is achieved through other different distributed FS like HDFS or Lustre.
Other options include Lustre and Ceph. %~\cite{yu2007exploiting} and Ceph%~\cite{donvito2014testing}.
%Lustre is a parallel file system ~\cite{yu2007exploiting} that presents high aggregated IO bandwidth by striping file extents across many storage devices. It provides fine-grained parallel file services with its distributed lock management. %Lustre separates essential file system activities into three components: clients, metadata servers, and storage servers.
%Ceph is an open source distributed storage system ~\cite{donvito2014testing},%  supported by Inktank Inc., designed to provide object, block and file storage in order to guarantee performance, reliability without single point of failure, fault tolerance by data replication and scalability to the exabyte level.
%\mara{Aggiungere qui due righe su cosa e' un datastore}
OpenNebula storage is structured around the \emph{Datastore} concept, \ie any storage medium to store disk images.
It makes use of a Datastore called Images, that points to the GlusterFS mount point, plus, other two (non replicated) datastores: \emph{System},  containing the instantiated machines data and \emph{Files \& Kernels} to store plain text files such as scripts.

%\begin{figure}[H]
%
%	\centering 
%	\includegraphics[width=6cm]{img/gluster.png}
%	\caption{Replicated Glusterfs Volume}
%	\label{gluster}
%	\label{fig:meth_env_gluster}
%\end{figure}
%

\subsubsection{Communication layer}
\label{sec:meth_env_comm}
In virtual environments, VMs are connected to virtual networks (VLANs) via virtual network interfaces. %More specifically, a VLAN definition consists of three different configurations, namely i)
%the underlying network infrastructure that will support it (e.g., the \emph{bridge}, explained in the following) and the network driver, ii) 	
%	its logical address space %(IPv4, IPv6, dual stack IPv4-IPv6 or Ethernet),
%	 iii) the guest configuration attributes, e.g., network masks, DNS servers or gateways.

IntraLAN communication refers to interactions among VMs in the same VLAN, while interLAN refers to cross VLAN communication.
The VLAN deployment and communications are managed in first instance by the IaaS platform.
The Layer 3 communication between different VLANs is made possible by \emph{Virtual routers} (VR), another type of VM that works just like a physical Layer 3 router, thus allowing for the definition of specific routing tables, gateways, etc.. A VR has one network interface in each VLAN that it manages.
However VMs might be deployed on different physical servers, therefore VLANs can span different nodes, that are in turn connected via physical switches. 
\emph{Virtual switches} are a key component in virtual environments, as they provide Hypervisors with connectivity between virtual interfaces of the VMs and the physical interfaces of the various nodes. 
They are software modules running on all nodes that maintain a MAC addresses database, to keep track of the VM addresses in the various LANs, process incoming input frames from physical interfaces and forward them based on the database. 

For the intraLAN and interLAN communication the two most commonly used virtual switches are \emph{Linux Ethernet Bridge} and \emph{Open vSwitch}.\\\\
%
%\paragraph{Linux Ethernet Bridge}
\textbf{Linux Bridge} is a layer 2 virtual device, integrated in Linux OS. It mainly consists of four major components: i) a set of managed physical interfaces, ii) a control plane managing the Spanning Tree Protocol (STP) (for network loops prevention), iii) a forwarding plane used to directs traffic to the appropriate interfaces based on mac address.\\\\
%
%\paragraph{Open vSwitch (OVS)} 
\textbf{Open vSwitch (OVS)} has been around since 2009 but hasn't been a contender to Linux Bridge before 2014. OVS provides the same functionality, plus other Layer3 functions. Licensed under the open Source Apache 2.0, it implements a virtual multilayer network switch, designed to enable effective network automation through programmatic extensions, while supporting standard management interfaces and protocols such as NetFlow, sFlow, SPAN, RSPAN, LACP and VLAN tagging.
%\sncs{In particular OVS supports the VXLAN protocol. VXLAN is a network virtualization scheme that enables users to create a logical network for virtual machines (VMs) across different networks. That is to say, it allows you to create a layer 2 network on top of layer 3 through encapsulation. What to emphasize is that you could potentially create 16 million networks using VXLAN, compared to the 4096 VLANs. In this case, VXLAN technology enables network to support far more VLANs. As a result, more logical network isolation for large networks can house much more virtual machines.}
OVS is used in multiple products and testing environments. 

\noindent Summing up the differences between the virtual switches, OVS is targeted at large multi-server virtualization environments, so it is focused on logical abstraction and management. The Linux bridge is fast and reliable, but lacks many control features.
IaaS like OpenStack and OpenNebula have started using OVS as default configuration in their networking framework. We also recommend the choice of OVS and assume this as a configuration choice in the following.

Multiple virtual switches (that in OVS are referred as \emph{bridges}) can be deployed to separate groups of VLANs logically, \eg internal lans versus others providing external services. 
Each VLAN is configured using the IaaS to sit on a single, specific bridge, as VMs receive their network address through the corresponding bridges (that, instead, have no address). 
%SILVIA: trovare un titolo migliore che renda l'idea che e' a supporto delle strati sopra
\subsubsection{Physical Infrastructure Configuration}
\label{sec:meth_phys_infrastructure}
Typically, the required physical infrastructure for the deployment of a Virtual Environment infrastructure consists of a number of physical servers (or \emph{nodes}), each one with its own specifications, and a number of physical switches, used to connect them (Figure~\ref{fig:meth_env_environment}). 
The servers run the IaaS software: in the particular case of OpenNebula, a ``master'' node must be configured to host the OpenNebula daemon, \emph{oned}, and the Sunstone Frontend, that communicates with oned, via \emph{XML-RPC} APIs. Other nodes just need to have the Hypervisor installed (package \texttt{opennebula-kvm} on Debian based systems). 

If OpenNebula's Image Datastore is managed via GlusterFS, the servers must be connected through a switch (we will call this the ``backbone'' network): when new templates containing VM datastores are added to the master node, the GlusterFS daemon will start file transfers to keep replicas updated.
To speed the sync between the replicas the bandwidth must be maximized. This translates to using high-end network interfaces on both the servers and the switch (i.e., use at least 10Gb ports).
If this is not possible, a bandwidth improvement can be made via \emph{interface bonding}.\\\\
\textbf{Linux bonding} driver provides a method for aggregating multiple network interfaces into a single logical "bonded" interface. In fact, the bonding allows combines several network interfaces into a single link, providing either high-availability, load-balancing, maximum throughput, or a combination of these. There are several bonding modes. One of them is mode 0 (balance-rr). In this mode, packets are transmitted in sequential order on the bond interfaces.\\
Furthermore, to enable VM communication via OVS bridges, the servers must be connected to a switch using one physical port per bridge. It is a good practice to use a separate switch for the backbone network and for OVS bridges, in order to physically separate business traffic pertaining to the emulated environment, and communication between the replicas.\\
All the logical pieces comprising the Emulation environment are resumed in Figure~\ref{fig:meth_env_environment}.

==> technical report/methodology_intro.tex <==

\section{Methodology}
%SILVIA: CHIACCHIERA
%idea di base della metodologia, cosa vogliamo andare a creare
%cloud based enviroment, physocal layer e; a supporto della virtual layer ma va consiferato.%
\label{sec:methodology}

In this section, we present a methodology for the design and deployment of a cloud-based emulation environment to support cyber-security testing, analysis and training activities.\\

\noindent The main goal of our methodology is to drive designers and system analysts in the creation of a virtualized environment that is able to reproduce a target networked physical environment, which will be used as a testbed.
The virtual environment will be deployed in a private cloud (leveraging IaaS frameworks) built on dedicated hardware.
%The sum of the virtual environment plus the physical environment will be called \emph{emulation environment}.
Our approach is articulated in three main activities: (i) \emph{Virtual Environment Infrastructure setup} (\ie how to set up a private cloud based on the physical infrastructure), (ii) \emph{Virtual Network Design} and (iii) \emph{Data Collection} from a deployed testbed.
We will use the term \emph{virtual} and \emph{emulation} environments interchangeably to refer to the enabling infrastructure and emulation/virtual \emph{testbed} to mean the reproduced network within it.\\

%Our approach is articulated along the following main phases:
\noindent {\bf Virtual Environment Infrastructure Setup.} This activity takes care of the design and deployment of the virtual environment on dedicated hardware. 
%\maraedit{
It is articulated along the following tasks: (a) select a cloud management platform to manage the storage and compute resources provided by the physical infrastructure, % (ii) a distributed storage must be selected in order to support flexibility, fast reconfiguration, and fault tolerance 
(b) define storage management policies for the virtual machines templates repository, in a way to foster data locality at instantiation time and fault tolerance and finally 
(c) design and deployment of the virtual communication infrastructure. 
%(iv) the integration of the previous task taking into account the physical resources available in the cloud.
Section \ref{sec:meth_env} discusses this activity, suggesting technological options to support each task.\\
%}

\noindent {\bf Virtual Network Design} This activity has the objective, starting from a reference network specification, to create a testbed configuration, \ie all the metadata needed to deploy its virtual counterpart. 
This can be done main in two ways: (i) by manually defining the characteristics of the required network or (ii) by gathering information from an existing network in order to clone it or use it as starting point. In the following, we will consider the second and most challenging case. %discussing the necessary steps to generate a virtual network starting from an an existing reference network. 
To this aim, we will discuss the following necessary tasks: (i) network topology identification,(ii) OS detection, and (iii) active service discovery in Section~\ref{sec:meth_ref_mapping}.\\
% discuss the details and options for each task.

\noindent {\bf Data Collection} This activity is responsible of ensuring proper handling of the experimental data (in the form of traffic captures) generated by the emulated testbed, %, so that can be properly analyzed at the end of each experiment. 
and is reported in Section~\ref{sec:meth_data_coll}.

%\begin{enumerate}
%\item \textbf{Emulation environment setup}: \silvia{Io direi piu' Private Cloud Setup}
%this phase takes care of the design, and deployment of an emulation environment on dedicated hardware. In particular, the choice of a cloud management platform, storage management policies and the configuration of the physical infrastructure will be discussed in Section~\ref{sec:meth_env}.

%\item \textbf{Reference network mapping}: is responsible of gathering information concerning the reference network that is to be replicated in the virtual environment. It is further divided in three sub-steps, \emph{network topology identification},\emph{OS detection}, and \emph{active service discovery}, detailed in Section~\ref{sec:meth_ref_mapping}. The outcome of this phase allows for the consolidation of the Virtual Environment Configuration. 
%\item \textbf{Data collection} this phase is responsible of ensure proper handling of the experimental data (in the form of traffic captures) generated by the emulated environment, so that can be properly analyzed at the end of each experiment. This procedure is reported in Section~\ref{sec:meth_data_coll}.
%\end{enumerate}
%see also Figure~\ref{fig:system_overview} for a pipeline overview.










==> technical report/methodology_mapping.tex <==


\subsection{Virtual Network Design}
\label{sec:meth_ref_mapping}
As previously stated, one of the objectives of an emulation environment is obtaining a separate, virtual and arbitrarily modifiable copy of an existing network for conducting analysis and tests.
In order to do that, fundamental inputs are the Network and Vulnerability Inventories and communication rules.
Such inputs are commonly available in large enterprise networks as they are  outputs of a continuous monitoring process and can be used to trigger cyber attacks detection and response processes. It is important to note that the effectiveness of the monitoring, detection and response activities depends on the accuracy of the collected inventories.\\\\
Inventory collection tools, such as GFI LANGUARD Network Scanner, typically require an intrusive approach, where monitoring agents are preinstalled on each host system. Furthermore, such as for the case of LANGUARD, they usually require expensive licenses. 
For these reasons in the following we will direct our choices towards software tools that are free and allow to perform this phase in a non intrusive way.\\

Instead, when this information is not available, such inputs can, in principle, be collected manually by interviewing a network administrator that lists all the requirements and details of the desired virtual network or by collecting them starting from a real physical network.

%In this section, we describe the necessary steps for mapping an actual real network to a virtual one, to be deployed in a virtual environment, namely i) network topology identification, ii) OS detection, and  iii) active service discovery \& vulnerability surface identification. For each step we also give an overview of the potentially helpful software tools and information.

 %As per our desiderata, we assume to have access to the least possible apriori available information.
%\mara{nell'introduzione mostriamo dei desiderata sulle scelte che prendiamo, esempio quella di non usare agents per il discovery}

\subsubsection{Network topology identification} This task allows to obtain a logic schema of the network infrastructure of the reference network in terms of ISO/OSI layers 2 and 3, i.e., of how many subnetworks it is composed, how they are separated using network devices (e.g., router, hubs, switches), as well as the presence of firewalls and their relative configuration rules.
%Note that concerning network devices, we are not here interested in the specific hardware brands and firmwares involved, as we will operate application level virtualization, that in this context refers to abstractions such as routing tables and firewall rules.

Common approaches for network discovery rely on distributed traceroute monitors~\cite{donnet2005improved}: however, the accuracy of this approach strongly depends on the observability of the network.

Overall, this phase is the hardest to automate, as in order to be accurate it relies heavily on pre-existing knowledge about the reference network, such as the one coming from Network Administrators and Network schemes. 

In the following, we make the assumption that the information about the number and composition of network LANS, as well as the network devices, is known a priori or can be determined by querying the network administrator. 
%In Section~\ref{meth_env_network} will be detailed how such information will be mapped to build the network topology for the emulated environment).

\subsubsection{Host and OS Detection}
\label{sec:meth_ref_osdetection}
Once that the network topology is known, an important step in the reference network mapping concerns identifying the computer hosts deployed in the network, to be able to replicate their presence in the virtual testbed.  
To this end, the primary information required is discovering active hosts on the network and their OS.\\\\
%This task (along with the identification of active ports, services, and applications~\cite{orebaugh2011Nmap}), is commonly referred as \emph{network scanning}. 
\emph{OS detection} is the process of determining the OS of a remote computer~\cite{orebaugh2011Nmap}. When this is accomplished in a non intrusive way (\ie, without deploying agents), it is achieved by  observing the external behavior of the remote host, mostly in terms of network traffic, in a way to derive what is called an OS \emph{fingerprint}~\footnote{a 67-bit signature describing the host behavior.}, adopting either an \emph{active} or an \emph{passive} approach.

Active OS fingerprinting requires sending specially crafted packet probes to the system in question, aiming at eliciting a distinguishable responses from different OS'es, derived from the implementation dissimilarities of their communication protocols~\cite{medeiros2009data}. %Probes include TCP and UDP packets that examine OS specifics such as initial sequence numbers (ISN), TCP options, IP identifier (ID) numbers, timestamps, explicit congestion notification (ECN), and window sizes~\cite{tyagi2015packet}. 
System responses from this active probing are then  used to generate the fingerprint and fed into a classification model.  Passive OS fingerprinting involves sniffing network traffic inside a network segment and matching known patterns to a table of pre-established OS identities. 
In general, active scanning allows for higher accuracy~\cite{richardson2010limits}, and passive is chosen only when a given degree of stealth or anonymity of capture is of concern%~\cite{matsunaka2013passive} 
(e.g., when aiming at performing malicious activities).

\paragraph{Tools}
The most popular active network scanner is Nmap~\cite{lyon2009Nmap}
, an open source tool designed for network exploration and security auditing. Nmap uses raw IP packets in novel ways to determine what hosts are available on the network, what services (application name and version) those hosts are offering, what OS version they are running, what type of packet filters/firewalls are in use, and dozens of other characteristics. Its output is composed of a list of scanned targets together with supplemental information on each, depending on the options used. %Usually, this information is a table of ports which lists the port number, protocol, service name, and state. 
Another tool offering OS detection capability is OpenVAS, most known for its value as a vulnerability assessment tool (see Section~\ref{sec:meth_service_vuln}).
%An example of passive TCP/IP stack fingerprinting tool is p0f~\cite{8406262}. %It sniffs traffic and uses a database of fingerprint descriptions to identify an OS~\footnote{It features also a Linux kernel level implementation called k-p0f that provides increased throughput, up to 450 kbps}.
Let us note that each of these tools has its own characteristics and main target applications. As a consequence, the produced output will satisfy different level of quality depending on the considered attributes. To improve the overall quality (in terms of accuracy of the scan operation) it is mandatory to integrate several scanners combining their output. Due to the lack of space, we postpone to Appendix~\ref{app:hybrid_approach} our proposal for combining results coming from Nmap and OpenVAS.

%\mara{TODO: Qui bisogna far passare il suggerimento: usare piu scanner e combinarne gli output per ottenere la migliore accuratezza. Noi suggeriamo di utilizzare Nmap + openvas, in appendice mostriamo un possibile flusso di integrazione dei due output}

%The components and subprocess of OS fingerprinting are presented in Figure 1 .
%\begin{figure}[H]
%	\centering 
%	\includegraphics[height=3cm, width=8cm]{img/os_detection.png}
%	\caption{OS fingerprinting process}
%	\label{os_detection}
%\end{figure}

\subsubsection{Active service discovery and vulnerability surface identification}
\label{sec:meth_service_vuln}
Determining what services are running on the network hosts is of primary importance to allow for an adequate mapping of the reference network.
In particular, for cyber security purposes, what is of interest is understanding the hosts' exposed ~\emph{vulnerability surface}, i.e. identifying which running services have an associated open port, and are thus, potentially directly exploitable.\\
A typical example is identifying DNS and HTTP servers are running and their respective versions. An accurate version number is key in determining which exploits a host is vulnerable to.\\
Vulnerability scanning tools usually produce a detailed report with the severity level of every vulnerability detected. %Nowadays, there are different vulnerability scanning tools, each one with specific characteristics. 
\paragraph{Tools}
OpenVAS is the open-source spin-off of the popular security scanner Nessus, and provides a modular architecture composed of a scanning agent and a manager with a powerful interface. The security scanner, is accompanied with a daily updated feed of Network Vulnerability Tests (NVT). 
% and it is free for Linux, Windows, and other operating systems. 
Being one of the most powerful free security scanners, supports thousands of vulnerabilities and offers false positive management of scanning results.
However, being a free tool it suffers from limitations with respect to its paid counterparts, such as Nessus, Nexpose or LANGUARD, such as limited DB, and cumbersome configuration.
Nmap is also capable of discovering open ports and associate services.
%Other common tools for service (and vulnerability) discovery are Nessus (commercial), GFI LANGUARD (commercial) and OpenVAS (free, opensource).
 

%\mara{TODO: Ovviamente puo integrare degli altri tool tipo LANGUARD per migliorare l'accuratezza, ma paghi}
 
%\paragraph{Port Scanning}
%Nmap's real power is its ability to efficiently scan ports. For a network connection to establish we need a port which is open at remote machine. Nmap offers a variety of port scan techniques, each with their own specific use and expected results. It is important to apply the proper scan technique to the environment and targets being scanned. Port scan type options are generally of the form -sC, where C is a prominent character in the scan name, usually the first \cite{lyon2009Nmap}.
%\begin{itemize}
%	\item \textbf{TCP SYN Scan (-sS)}\\
%	By default, Nmap performs a TCP SYN scan (-sS) against the specified target, when run with root or administrator privileges. SYN scanning is quick and provides reliable results for open, closed, and filtered ports.
%	\item \textbf{TCP Connect Scan (-sT)}\\
%	If a user doesn't have root or administrator privileges, Nmap will perform the TCP connect scan (-sT ) by default. This is because Nmap uses the underlying OS to establish a connection with the target instead of using its built-in ability to create and send raw packets. This scan method tends to be less efficient since Nmap has less control than it does when creating raw packets.
%	\item \textbf{TCP NULL Scan (-sN), TCP FIN Scan (-sF), Xmas Scan (-sX)}\\
%	According to the TCP RFC, any packet not containing a SYN, RST, or ACK flag will result in a returned RST if the port is closed and no response if the port is open. Nmap includes other three scan options to take advantage of this characteristic. TCP Null scan (-sN ) does not set any flag bits in the TCP header. TCP FIN scan (-sF ) sets only the FIN flag. Xmas scan (-sX ) sets the FIN, PSH, and URG flags.
%	\item \textbf{TCP ACK Scan (-sA)}\\
%	This scan method is used to map out firewall rulesets (i.e. determining whether they are stateful or not and which ports are filtered). By default, the ACK scan probe has only the ACK flag set.
%	\item \textbf{UDP Scan (-sU)}\\
%	Although the most popular services on the Internet run over the TCP protocol, there exist UDP services which are widely deployed, e.g. DNS, SNMP, and DHCP. Then, Nmap offers the option of a UDP scan with the -sU option. UDP scanning can be combined with a TCP scan type, such as SYN scan (-sS), to check both protocols during the same run.
%\end{itemize}
%For our network scan we have used only the -sS scan since we had root privileges. We avoided using the UDP scan, since it is very slow for a medium network.


%Nmap provides the -sV option for enabling version detection. Version detection works by interrogating those TCP or UDP ports flagged as open or open|filtered during the port scanning phase, with the purpose of identifying the software version that is actually running on those particular ports.\\


\subsubsection{Testbed Configuration}
In this section we summarize the metadata needed in order to deploy our testbed, derived from the phase of Virtual Network Design. It is composed of \emph{Hosts configuration} and \emph{Network configuration}, consolidated in the Testbed Configuration (Figure ~\ref{fig:system_overview}).\\\\
\textbf{Hosts Configuration} Each host identified from the reference network is associated to an OS template in the Images Datastore, a list of installed services CPE (with optional version) and a list of network interfaces. Optionally, a host-specific synthetic behavior can be embedded by deploying appropriate software code (see for example Section~\ref{sec:dataset_generators}).\\\\\textbf{Network Configuration} All network LANS will have a corresponding VLAN configuration, assigned to OVS Bridges also based on the data collection requirements (see Section~\ref{sec:meth_data_coll}). All layer 3 network devices will have a corresponding Virtual Router configuration, with their corresponding interfaces (see Section~\ref{sec:meth_env_comm}), physical Firewalls will correspond to Virtual Firewalls.

This information may be stored in a database or other means, if automation of the deployment is of concern. Most IaaS platforms offer their APIs to allow for automation of deployment to various extents. OpenNebula offers a centralized XML-RPC interface that can be used to entirely manage the emulated testbed in an automatic way, such as creating VLANs, instantiating VMs, etc. In Section~\ref{sec:case_study} can be found an example on how to fully automate the deployment of a test environment using OpenNebula API. 




==> technical report/related_work.tex <==
%!TEX root = ./main.tex
\section{Related Work}


\mara{TODO: Qui io parlerei del progetto PANOPTESEC}

\paragraph{Tools for creating emulated environments}

\mara{Terraform}
In~\cite{eskridge2015vine} the authors proposed a Virtual Infrastructure for Network Emulation (VINE), pointing out for a set of tools that helps the construction of virtual topologies allowing for different type of experiments for cyber security researchers. %In particular, they provide three topology-generation methods: manual, programmatic, and tool-based. 
Furthermore, VINE supports traffic behavior generation using monitored agents or the traditional packet capture for a low-level analysis of the state of the hosts. Operators can exploit a web-based interface, to manually create, modify, and monitor experiment testbeds as well as a JSON HTTTP interface for automated generation and control experiments. The main drawback of this paper is that the platform is overviewed at a rather general viewpoint, without allowing for a deep comparison.

\sncs{As cybersecurity work, the authors in ~\cite{Pham2016CyRISAC} proposed a Cyber Range Instantiation System (CyRIS). It is a solution of reliably and repeatably creating and managing environments for cybersecurity training courses. In particular, CyRIS is an automated tool that takes a cyber range definition description (a file)and creates the desired training environments without human interaction. Furthermore, it supports both basic features for preparing the infrastructure, and security features for configuring sophisticated security related content.}

\paragraph{Mapping a reference environment}
%[Raniero]'s paper 
All considered tools provide means for security testbeds instantiation and experimentation, and either concentrate on Most papers concentrate either of . Our work documents instead a complete end-to-end methodology mapping an existing real environment inside an emulated environment, and performing cyber security experiments.
Previously, ~\cite{raniero18} Rapone et al. concentrated of the latter aspect, on providing a measurable metric for determining the affinity of a virtual environment with respect to the reference real environments.
\mara{Il paper di Raniero sembra piu un technical report (non pubblicato, presente solo su researchgate). Valutiamo se ometterlo.}



%\paragraph{Works on Network intrusion dataset collections}
We refer to more related work in each of the following sections.

==> technical report/study_case.tex <==

\section{A Case Study: DIAG Department}
\label{sec:case_study}
As a candidate for a case study, we chose the network of the Department of Computer, Control, and Management Engineering Antonio Ruberti (DIAG).
In particular, we followed the methodology described in Section~\ref{sec:methodology} and set up an emulation environment based on OpenNebula, using OVS for the connection layer, and GlusterFS for mantaining a replicated Images Datastore, and deployed an emulated testbed.

The network topology of the department consists of seven subnets, that we will call LAN1, LAN2, LAN3, LAN4, CED, DMZ\_INT and DMZ\_EXT.
The first three contain personal workstations (with a few exceptions of servers) of research staff belonging to various research areas, like Computer Science, Automation and Control and Management Engineering and the fourth pertains to administrative staff.
Furthermore, CED contains servers and compute nodes used by researchers to perform their work, while DMZ\_INT hosts internal services, such as SMB or SFTP and finally DMZ\_EXT hosts servers that expose services towards Internet (such as a WWW server and an SVN repository).

The following sections discuss each implementation step of the methodology in the context of this case study.
\subsection{OS Detection and Vulnerability Discovery}
We performed OS detection following the hybrid approach of Appendix~\ref{app:hybrid_approach} after executing Nmap and OpenVAS scans of each LAN.
Figure~\ref{fig:study_case_os_detection} shows the distribution of the different OS Families for each LAN, fot a total of 215 hosts.
\begin{figure}[H]
	\centering 
	%left low right up
	\includegraphics[width=0.7\linewidth,trim={2.5cm 3.75cm 2.5cm 3cm},clip]{img/detection.pdf}
	\caption{OS Detection results.}
	\label{fig:study_case_os_detection}
\end{figure}
%48 Windows
%41 Other 
Since we are interested in mapping each host to a VM Template, we need accuracy at the OS Generation level.
Excluding all entries belonging to the \emph{Other} Family (mostly network devices, firewalls, access points, etc.), we could unambiguously determine the OS Generation for about 60\% of the host virtual machines, while relying solely on Nmap we could map only about 25\% (mostly corresponding to Windows machines, for the reasons expressed in Section~\ref{sec:meth_ref_osdetection}, while with OpenVAS alone we reached 45\% overall. Unfortunately, due to problems with the KVM Hypervisor, we couldn't manage to emulate correctly the OSX Machines, and resorted to only keeping Windows and Linux VMs (the specific OS Generations will be detailed in the following).

%Unfortunately, for these mappings we can provide accuracy results onlu for DMZ andCED AREA, as we could obtain the ground trugh information from the network admin. For that specific sample, the hybrid technique gave almost the same results of OpenVAS alone.

%In this case OpenVAS helped us to improve and/or complete those cases that are misidentified from using Nmap only. The tools increase the degree of accuracy to 95\%. Furthermore, for some LANs (CED, DMZ\_INT and DMZ\_EXT) we could compare the results with a ground truth provided by the network administrator.  As shown in the figure above, each LAN has not only a different distribution in terms of OS Detection but also by the number of discovered hosts. The number of hosts with the relative OS are dependent on the type of LAN, since each of them covered a particular area of teachers/researchers (algorithm, robotic, etc). LANs with only OS Linux hosts is normal for the LANs with the servers or exposed internal/external services. On the other hand, LAN with a majority number of host with Linux OS is probably preferred in a area with pure computer scientist.
  
OpenVAS and Nmap were also implied in the discovery of running services as well the known vulnerabilities for each host. 
%Practically, we collected all version for each one in order to have the right version with the same vulnerability. The applications that were not identified by OpenVAS are installed with the last version released. For the followings LANs we have found the corresponding top services.
Figure~\ref{fig:study_case_top_services} reports the top occurring services found in the various LANs.
\begin{figure*}
	\centering 
	%left low right up
	\includegraphics[width=1.15\linewidth,trim={0.1cm 16.cm 0cm 0cm},clip]{img/top_services.pdf}
	\caption{Top 5 installed services by percentage of installations in the various LAN of the reference network.}
	\label{fig:study_case_top_services}
\end{figure*}

\subsection{Physical infrastructure}
%The construction of emulated environment is based on the underlying physical infrastructure. It includes different hardware parts and in our case we needed to set up them with specific configurations. 
Table~\ref{tab:study_case_testbed_conf} reports hardware configuration of our Virtual Environment infrastructure.
\begin{table}[]
\centering
	\caption {Hardware Specifications}
	\begin{tabular}{|c|c|l|}
		\hline
		\multicolumn{1}{|c|}{\textbf{Type}} & \multicolumn{1}{c|}{\textbf{Name}}                                            & \textbf{Specifications}                                                                                                                                                                 \\ \hline
		Server                     & \begin{tabular}[c]{@{}c@{}}$2 \times$ Cisco UCS C240\\ M4S\end{tabular} & \begin{tabular}[c]{@{}l@{}}- $2 \times$ Intel Xeon E5-2620v3\\ (24 total threads)\\- 64 GB RAM\\ %- 10 x 1GB ports\\ - 2 x 10GB ports\\ 
		- 8 x HDD 1.2 TB\end{tabular} \\ \hline
		\multirow{2}{*}{Switch}    & Cisco Catalyst 2960XR                                                & \begin{tabular}[c]{@{}l@{}}%- Switch layer L2\\
		 - APM86392/512 MB RAM\\ - 48 x 1GB Ports \\\end{tabular}                                                                \\ \cline{2-3} 
		& Cisco Catalyst  WS-C3850                                             & \begin{tabular}[c]{@{}l@{}}%- Switch layer L3\\ 
		 - MIPS/4 GB RAM\\- 24 x 10GB Ports\\\end{tabular}                                                                       \\ \hline
	\end{tabular}
	\label{tab:study_case_testbed_conf}
\end{table}
The two servers, connected via the L2 switch Cisco Catalyst 2960 form the backbone network for GlusterFS traffic, while the second L3 Cisco Catalyst WS-C3850 switch is used for the emulation environment (OVS bridges)%~\footnote{Even if not technically needed for this 2-server configuration, the switches have been implied both for sake of generality and as we have plans to expand our network in the immediate future}.
As detailed in the following, we will make use of 3 OVS bridges for networking.
Each bridge uses a physical network interface on each server. %to support the physical communication between the servers on different VLANs. %These are created following a specific design that will be showed in the next section.  
The basic templates for the VMs and the ISO Images for the various operating systems are saved in the Image Datastore. 
Since we couldn't count on high performance Ethernet interfaces on the nodes, we adopted the Linux bonding strategy to maximize the bandwidth on the backbone network. In particular, we used Linux kernel bonds with bond-mode 0, and 6 1GBps interfaces per node, achieving in this way a maximum bandwidth equal to 6 Gbps.

%The virtual environment is designed to have different virtual networks where virtual machines communicate through intraLAN and/or interLAN communication. For these communications layer we used Open vSwitch as virtual switch, as already specified in the methodology, where we defined all the VLANs.
 
%\begin{figure}[H]
%	\centering 
%	\includegraphics[width=1\linewidth]{img/schema_switch.pdf}
%	\caption{Physical Architecture Layout}
%	\label{fig: physical}
%\end{figure}
%In the figure above are shown the physical configuration of the components, in particular the wired communications. They are configured as follows:
%\begin{itemize}
%	\item Bonding: 6 network interfaces for each server ( yellow and blu cables).
%	\item Open vSwitch: 3 interface for bridge br1, br2 and br3 (green cables).
%\end{itemize} 
\subsection{Testbed Architecture}
\label{sec:studycase_testbed}

Due to lack of resources, and also considering other VMs necessary for networking, firewalling and generation of benign and malicious background traffic by external hosts, we could only afford to instantiate about half of the identified host machines.
%To reflect the reference network, we designed and implemented different networks on OpenNebula.
We deployed all the VLANs necessary for replicating the reference network, using three OVS virtual bridges, namely \texttt{br1, br2 and br3}. The first bridge will be devoted to internal, business LANs, the second to service-related VLANs, and network devices (routers and a firewall), while the third bridge provides Internet connection to the whole testbed hosting the interfaces of all such machines that need direct internet connection.

For VLAN Routing at Layer3, we made use of three Virtual Routers, namely VR0, VR1 and VR2. Furthermore, as per the reference network, we use a Virtual Firewall, \emph{FW}. Virtual Routers run ZeroShell v3.8.2, a lightweight Linux Distribution suited 
for router emulation. For the firewall, we used PfSense 2.4.3.\\

%\sncs{Nowadays, there are three main Open Source Firewalls: Untagle, Pfsense, Ipfire. By a brief comparison of them, pfSense was the best solution that met our objectives. Pfsense is a firewall ~\cite{patel2017review,} on FreeBSD operating system such as, a comprehensive network security solution which integrates all of the security services such as firewall, URL filtering, virtual private networking etc in a single appliance.}
%As firewalls, there are more than one solution as virtual router. Zeroshell is a Linux based distribution  dedicated to the implementation of Router and Firewall Appliances completely administrable via  web interface. Zeroshell is available for x86/x86-64 platforms and ARM based devices such as Raspberry Pi. Some advanced features of Zeroshell are: load balancing and failover of multiple internet connections, VPN site to site and VPN host to site and captive portal access for internet hotspot [citare pagina web].
\noindent More specifically, the architecture is divided in the following parts:\\
\textbf{Internal Area:} This area is composed by LAN1, LAN2, LAN3 and LAN4. The virtual networks are available to the virtual machines through the corresponding bridge \texttt{br1}. \\
\noindent	\textbf{DMZ Area:} CED and DMZ\_INT provide internal services to authorized hosts in the Internal Area through VR1. DMZ\_EXT contains servers exposing services to the Internet. Note that access to services in the DMZ area is allowed by well defined firewall rules specified on FW.\\
\noindent	\textbf{External Hosts:} This VLAN, as well as Attackers, is used to simulate a portion of the Internet, made by hosts that will connect to services from the DMZ\_EXT VLAN.\\
\noindent	\textbf{Attackers:} The Attackers network, hosts  malicious external attackers that want to exploit or attack hosted services (Section~\ref{sec:attack_scenarios}). %For instance, they can connect to the public services in the DMZ\_EXT area though VR2. 

DMZ Area, Attackers and External Hosts VLANs are deployed on bridge br2.
Table~\ref{tab:study_case_testbed_network} summarizes the list of VLANs, networks addresses and number of hosts, with installed operating systems and related public and private IPs and services installed in the service LANs. 
Note that both External Hosts, Attackers and servers in the DMZ\_EXT have ranges in the public IPv4 space: indeed we replicated a small portion of the internet inside our testbed. 

In order for the communication from such networks to correctly reach the DMZ\_EXT (instead of flowing towards the Externet VLAN), a static route was configured on VR2 to direct traffic with destination inside DMZ\_EXT through VR2's interface on FWVR2. 

Thus, traffic from such external hosts directed to DMZ\_EXT
will be routed by VR2, using the static route, and all the corresponding responses will return back to the originating hosts, since VR2 knows both External Hosts and Attackers through direct interfaces.\\ 

%The Internal Area consists of four VLANs with 37 hosts with private IPs and includes different operating systems Windows and Linux in general.
%The DMZ Area includes three VLANs. CED and DMZ\_INT have eight hosts with private IPs which have Ubuntu and OpenSUSE as OS family versions. DMZ\_EXT has only two hosts and exposes to Internet, thus public IP, a Drupal site and a server (heartbleed). External Hosts and Attackers VLANs contains respectively three and two hosts with public IPs. In particular, Attackers contains two Kali Linux virtual machines.
\begin{figure*}
	\centering 
	\includegraphics[width=1\linewidth]{img/testbed_services.pdf}
	\caption{Testbed network architecture: The VLANs arrangement in L2 OVS bridges is highlighted using blue boxes. Installed services on service LANs are also shown. Reported package versions were automatically installed in the testbed, original ones from the reference network are in parentheses.}
	\label{fig:study_case_testbed_architecture}
\end{figure*}

\begin{table}
\centering
	\caption {LANs Operating Systems and IPs}
	\begin{tabular}{|c|c|l|l|}
		\hline
		\textbf{LAN}              & \textbf{Network}                                                                  & \textbf{OS}                                             & \textbf{IPs}                                                               \\ \hline
		\multirow{8}{*}{LAN1}     & \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{10.1.10.}0/24\\ 20 hosts\end{tabular}}  & Ubuntu 12.04                                            & 16                                                                        \\ \cline{3-4} 
		&                                                                                   & Ubuntu 14.04                                            & 4, 22                                                                    \\ \cline{3-4} 
		&                                                                                   & Ubuntu 16.04                                            & \begin{tabular}[c]{@{}l@{}}6-10, 13\\15, 17, 19\end{tabular}      \\ \cline{3-4} 
		&                                                                                   & Ubuntu 16.10                                            & 18                                                                        \\ \cline{3-4} 
		&                                                                                   & Debian 7                                                & 12                                                                        \\ \cline{3-4} 
		&                                                                                   & Windows 10 (1803)                                   & 11, 14                                                                   \\ \cline{3-4} 
		&                                                                                   & Win. Server 2008 SP1                                 & 21                                                                        \\ \cline{3-4} 
		&                                                                                   & Win. Server 2012 R2                                  & 20                                                                        \\ \hline
		\multirow{4}{*}{LAN2}     & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{10.1.11.}0/24\\ 5 hosts\end{tabular}}   & Ubuntu 16.04                                            & .3                                                                         \\ \cline{3-4} 
		&                                                                                   & Windows 7                                               & 6                                                                         \\ \cline{3-4} 
		&                                                                                   & Windows 10 (1709)                                   & 5                                                                         \\ \cline{3-4} 
		&                                                                                   & Windows 10 (1803)                                   & 2, 4                                                                     \\ \hline
		\multirow{5}{*}{LAN3}     & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{10.1.8.}0/24\\ 8 hosts\end{tabular}}    & Ubuntu 14.04                                            & .6                                                                         \\ \cline{3-4} 
		&                                                                                   & Windows 7 SP1                                           & 2, 4                                                                     \\ \cline{3-4} 
		&                                                                                   & Windows 10 (1709)                                    & 5                                                                         \\ \cline{3-4} 
		&                                                                                   & Windows 10 (1803)                                   & \begin{tabular}[c]{@{}l@{}}3, 7, 9\end{tabular}                       \\ \cline{3-4} 
		&                                                                                   & Win. Server 2008 SP1                                 & 8                                                                         \\ \hline
		\multirow{4}{*}{LAN4}     & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{10.1.12.}0/24\\ 4 hosts\end{tabular}}   & Windows 7                                               & 2                                                                         \\ \cline{3-4} 
		&                                                                                   & \begin{tabular}[c]{@{}l@{}}Windows 7 SP1\end{tabular} & 3                                                                         \\ \cline{3-4} 
		&                                                                                   & Windows 10 (1709)                                    & 5                                                                         \\ \cline{3-4} 
		&                                                                                   & Windows 10 (1803)                                   & 4                                                                         \\ \hline
		\multirow{2}{*}{CED}      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{10.2.20.}0/24\\ 4 hosts\end{tabular}}   & Ubuntu 10.04                                            & 5                                                                         \\ \cline{3-4} 
		&                                                                                   & Ubuntu 16.04                                            & 2-4                                                                       \\ \hline
		DMZ\_INT                  & \begin{tabular}[c]{@{}c@{}}\textbf{10.2.9.}0/24\\ 4 hosts\end{tabular}                     & OpenSUSE 11.4                                           & 2-5                                                                       \\ \hline
		\multirow{2}{*}{DMZ\_EXT} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{200.100.0.}0/26\\ 2 hosts\end{tabular}} & Ubuntu 14.04                                            & 8                                                                         \\ \cline{3-4} 
		&                                                                                   & Ubuntu 16.04                                            & 3                                                                         \\ \hline
		Ext. Hosts                & \begin{tabular}[c]{@{}c@{}}\textbf{80.}0.0.0/8\\ 3 hosts\end{tabular}                      & Ubuntu 16.10                                            & \begin{tabular}[c]{@{}l@{}}20.40.2,\\ 100.3.50,\\ 20.55.21\end{tabular} \\ \hline
		Attackers                 & \begin{tabular}[c]{@{}c@{}}\textbf{1.2.3.}0/27\\ 2 hosts\end{tabular}                      & Kali Linux 4.15.0                                              & 2, 16                                                                    \\ \hline
	
	\end{tabular}
	\label{tab:study_case_testbed_network}
	\end{table}
	
	
	
	
\noindent \emph{Testbed deployment} The deployment of all VLANS, VMs, Virtual Routers and Firewall components was completely automated using a Python based module via the Python bindings of the XML-RPC APIs exposed by OpenNebula. 
%VMs have been deployed using the \texttt{template.instantiate} API, specifying OS templates. 
%The templates have been created before the deployment, taking in consideration the output of the OS Detection. We could not replicate all the operating systems and completely the number of hosts from the reference network. For hardware resources reasons we deployed only a specific number of hosts for each LAN. Furthermore, we omit to deploy the Mac OS X hosts since they have difficulties with the KVM hypervisor.

In order to provide each machine with the appropriate services (with version) determined in the vulnerability surface identification phase, we created startup scripts according to each operating system family, that we feed with the services to be installed, so that they are fetched and installed automatically at first machine boot.

A particular effort must be devoted for the installation of the services, starting from the CPEs. Currently, there is no available data source that allows to match application CPEs to actual packages. 
For this reason the mapping must resort to either a manual association, or a tentative automatic association based on similarity. 

In particular, we resorted to manually mapping application CPE to software packages, that then were installed automatically using the closest version available in the repositories.
%\begin{table}[]
%	\begin{tabular}{|c|c|c|l|}
%		\hline
%		\textbf{LAN}                                    & \textbf{IP}                      & \textbf{Name} & \textbf{Services}                                                                                                                          \\ \hline
%		\multirow{4}{*}{CED}                            & 10.2.20.2                        & ced1          & openssh:7.2p2                                                                                                                              \\ \cline{2-4} 
%		& 10.2.20.3                        & ced2          & openssh:7.2p2                                                                                                                              \\ \cline{2-4} 
%		& 10.2.20.4                        & ced3          & openssh:7.2p2                                                                                                                              \\ \cline{2-4} 
%		& 10.2.20.5                        & ced4          & \begin{tabular}[c]{@{}l@{}}openssh:7.2p2\\ apache2:2.2.14\end{tabular}                                                              \\ \hline
%		\multirow{4}{*}{DMZ\_INT}                       & 10.2.9.2                         & lsrv          & \begin{tabular}[c]{@{}l@{}}openssh:6.6.1p1\\ tightvnc:1.3.9(1.2.9)\\ samba:3.6.3\end{tabular}                                              \\ \cline{2-4} 
%		& 10.2.9.3                         & int1          & \begin{tabular}[c]{@{}l@{}}openssh:6.6.1p1(5.1)\\ tightvnc:1.3.9 (1.2.9)\\ vsftpd:2.0.7\end{tabular}                                        \\ \cline{2-4} 
%		& 10.2.9.4                         & int3          & \begin{tabular}[c]{@{}l@{}}openssh:6.6.1p1(4.2)\\ tightvnc:1.3.9 (1.2.9)\\ xorg:1.6.5\end{tabular}                                         \\ \cline{2-4} 
%		& 10.2.9.5                         & int2          & \begin{tabular}[c]{@{}l@{}}openssh:6.6.1p1(5.1)\\ tightvnc:1.3.9 (1.2.9)\end{tabular}                                                       \\ \hline
%		\multicolumn{1}{|l|}{\multirow{2}{*}{DMZ\_EXT}} & \multicolumn{1}{l|}{200.100.0.3} & www           & \begin{tabular}[c]{@{}l@{}}drupal:7.1\\ mysql:5.5.54(5.7.22)\\ openssh:7.2p2(6.6.1)\\ apache2:2.4.18(2.2)\\ php:5.6.36(5.3.17)\end{tabular} \\ \cline{2-4} 
%		\multicolumn{1}{|l|}{}                          & 200.100.0.8                      & svn           & \begin{tabular}[c]{@{}l@{}}apache2:2.4.7(2.2.10)\\ openssh:6.6.1p1(5.1)\\ mysql:5.5.54(5.7.22)\end{tabular}                                 \\ \hline
%	\end{tabular}
%	\caption{Installed services on the server in CED, DMZ\_INT and DMZ\_EXT. The listed package versions are those automatically installed in the testbed, while the  ones originally present in the reference network are shown in parentheses.}.
%	\label{tab:study_case_server_services}
%\end{table}
%\subsubsection{Appendice Nmap-OpenVAS}
%\sncs{In general OS Detection is a process where both Nmap and OpenVAS needs to have a ground truth in order to validate the obtained results. As already specified Nmap provides different osmatch according to accuracy level. In particular, for some hosts it gives as output only a one osmatch or more than one with the best accuracy. In order to test the OS Detection goodness, we compared the results provided from Nmap with a ground truth of the LANs CED, DMZ\_INT and DMZ\_EXT for which we have both the OS family and OS generation. We considered as correct result those cases in which Nmap provides two or more OS generations but among them it identified the right one (ground truth). From a list with 26 hosts, Nmap identified with an accuracy of 100\% all the hosts OS Family. However, Nmap does not provide the distribution of a determined OS Family for Linux (i.e. Ubuntu) but only the kernel version. Therefore, in this case the Nmap accuracy was only of 7\% in terms of OS generation detection.
%We also tested the goodness of OpenVAS, considering both OS family and OS generation. As opposed to Nmap, OpenVAS when it is possible detects the distribution for the Linux hosts. However, sometimes OpenVAS does not return any information about OS (Family or/and Generation). For the test we considered as Nmap case all the 26 hosts in the three LANs. In our case, the OS family of all the hosts was correctly detected, thus it has a 100\% degree of accuracy. For the OS Generation OpenVAS provide a good improvement compared to Nmap. Indeed, it provides correct OS generation detection with an accuracy of 45\%.
%Our approach considered both of them, since each tool provide complementary detections that the other tool did not provide. Using Nmap and OpenVAS together, in the case of LANs with the available ground truth, we have a final 50\% of accuracy for the OS generation.}      

